Earthquake theorem for cluster algebras of finite type

We introduce a cluster algebraic generalization of Thurston's earthquake map for the cluster algebras of finite type, which we call the \emph{cluster earthquake map}. It is defined by gluing exponential maps, which is modeled after the earthquakes along ideal arcs. We prove an analogue of the earthquake theorem, which states that the cluster earthquake map gives a homeomorphism between the spaces of $\mathbb{R}^\mathrm{trop}$- and $\mathbb{R}_{>0}$-valued points of the cluster $\mathcal{X}$-variety. For those of type $A_n$ and $D_n$, the cluster earthquake map indeed recovers the earthquake maps for marked disks and once-punctured marked disks, respectively. Moreover, we investigate certain asymptotic behaviors of the cluster earthquake map, which give rise to "continuous deformations" of the Fock--Goncharov fan.

==> 6_asymp_old.tex <==
\section{Asymptotic behavior of the images by the earthquake maps of the cluster complexes}\label{sec:asymptotics}

For a point $g_0 \in \cX_\bs(\pos)$, the set of intersections of the subsets $\cD^+_{(v)}(g_0)$, $v \in \bExch_\bs$ is a simplicial set but not a fan in $\log \mathbf{X}^{(v_0)}(\cX_\bs(\pos))$ for any $v_0 \in \bExch_\bs$. 
Namely, the simplices are not cones, in other words, they are not invariant under the $\pos$-action.
(Roughly speaking, the simplicies are not linear.)
%Although, 
Nevertheless, we are going to see that the set is a fan at the \emph{Thurston boundary} of $\cX_\bs(\pos)$ in a certain sense.

The subsets $\cD^+_{(v)}(g_0)$ are defined by the image $E(g_0, L)$ of the points $g_0 \in \cX_\bs(\pos)$ and $L \in \cX_\bs(\bR^\trop)$ by the earthquake map $E: \cX_\bs(\pos) \times \cX_\bs(\bR^\trop) \to \cX_\bs(\pos)$.
Taking the limit $L \to \infty$ for $E(g_0, L)$, then this point goes to the boundary of $\cX_\bs(\pos)$.
We will this direction in \cref{subsec:L_to_infty}.
On the other hand, one can take the limit $g_0$ to the boundary of $\cX_\bs(\pos)$ for $E(g_0, L)$.
We will see this direction in \cref{subsec:g_to_infty}.
% In \cref{subsec:L_to_infty}, we will consider the set defined by taking the limit $L \to \infty$ for $E(g_0, L)$, and in \cref{subsec:g_to_infty}, we will consider the limit $g$ to the boundary of $\cX_\bs(\pos)$ for $E(g_0, L)$.

\subsection{The case of $L$ to infinity}\label{subsec:L_to_infty}
Let us fix a mutation class $\bs$ of finite type, a point $g_0 \in \cX_\bs(\pos)$ and a vertex $v_0 \in \bExch_\bs$.
Let us consider the plot $\log \mathbf{X}^{(v_0)} \circ E(g_0,-):\X_\bs(\bR^\trop) \to \bR^I$ of the cluster earthquake map in the log-coordinate associated with $v_0$. Although the image of each cone of the cluster complex is very different from the plot of the corresponding cluster complex (see the proof of \cref{lem:homeo_rank2}), we observe that the plot \cref{fig:log_earthquake_far} seen from a distance looks similar to the plot \cref{fig:cluster_complex_minus} of the cluster complex of the opposite $-\bs$ of the given mutation class $\bs$.
(See \cref{def:opposite} for the definition of the opposite mutation class.)


% Namely, $-\bs$ is the mutation class such that there is a graph isomorphism
% \begin{align*}
%     \bExch_\bs \xrightarrow{\sim} \bExch_{-\bs}\,;\quad v \mapsto -v
% \end{align*}
% satisfying $\varepsilon^{(-v)} = -\varepsilon^{(v)}$ for all $v \in \bExch_\bs$.

One can verify that there is a PL isomorphism 
\begin{align}\label{eq:iota}
    \iota: \cX_\bs(\bR^\trop) \xrightarrow{\sim} \cX_{-\bs}(\bR^\trop)
\end{align}
such that $x_i^{(-v)}(\iota(L)) = -x_i^{(v)}(L)$
for each $v \in \bExch_\bs$ and $L \in \cX_\bs(\bR^\trop)$
%Namely, the relation \eqref{eq:X_i^(-v)} is compatible with the coordinate transformations (\emph{i.e.}, tropicalized cluster transformations)
\footnote{One can verify that there is an isomorphism $\iota: \cX_\bs(\pos) \xrightarrow{\sim} \cX_{-\bs}(\pos)$ in the same way.}.
% \begin{itemize}
%     \item for $\bA=\pos$ and any $g \in \cX_\bs(\pos)$, and
%     \item $x_i^{(-v)}(\iota(L)) = -x_i^{(v)}(L)$ for $\bA = \bR^\trop$ and any $L \in \cX_\bs(\bR^\trop)$.
% \end{itemize}
We will identify $\cX_\bs(\bR^\trop)$ and $\cX_{-\bs}(\bR^\trop)$ by this isomorphism $\iota$.

\begin{figure}[h]
    \centering
    \begin{tikzpicture}
    \node at (0,0) {\includegraphics[width=4cm]{A2_D_25.png}};
    \node at (5,0) {\includegraphics[width=4cm]{B2_D_25.png}};
    \node at (10, 0) {\includegraphics[width=4cm]{G2_D_25.png}};
    \node at (0,-2.5) {$A_2$};
    \node at (5,-2.5) {$B_2$};
    \node at (10,-2.5) {$G_2$};
    \end{tikzpicture}
    \caption{The images $\log \mathbf{X}^{(v_0)} (E(g^{(v_0)}_1, \cC^+_{(v)}))$ of the cones $\cC^+_{(v)}$, $v \in \bExch_\bs$. These plots are drawn in more wide range (explicitly, the range is $[-25, 25] \times [-25, 25]$) than the figures in the proof of \cref{lem:homeo_rank2}.}
    \label{fig:log_earthquake_far}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{tikzpicture}
    \node at (0,0) {\includegraphics[width=4cm]{A2_C_minus.pdf}};
    \node at (5,0) {\includegraphics[width=4cm]{B2_C_minus.pdf}};
    \node at (10, 0) {\includegraphics[width=4cm]{G2_C_minus.pdf}};
    \node at (0,-2.5) {$A_2$};
    \node at (5,-2.5) {$B_2$};
    \node at (10,-2.5) {$G_2$};
    \end{tikzpicture}
    \caption{The cluster complex of the opposite mutation class $-\bs$.
    Namely, the cones $\mathbf{x}^{(v_0)}(\iota^{-1}(\cC^+_{(-v)}))$ in $\bR^I$.}
    \label{fig:cluster_complex_minus}
\end{figure}

%In this subsection, we will see the images of the cones $\cC^+_{(v)}$ by $\log \mathbf{X}^{(v_0)} E_\bullet(g_0)$ in the boundaries of the cluster manifolds $\cX_\bs(\pos)$.
In order to formulate our observation on the plot ``seen from a distance'', let us recall the \emph{Thurston compactification} $\overline{\cX_\bs(\pos)}$ of a cluster manifold $\cX_\bs(\pos)$ \cite{Le16,FG16,Ish19}. It is given by the spherical compactification
\begin{align*}
    \overline{\cX_\bs(\pos)} := \cX_\bs(\pos) \sqcup \bS \cX_\bs(\bR^\trop)
\end{align*}
where $\bS \cX_\bs(\bR^\trop) := (\cX_\bs(\bR^\trop) \setminus \{0\}) / \pos$.
It is endowed with a topology such that a divergent sequence $g_n$ in $\cX_\bs(\pos)$ converges to $[L] \in \bS \cX_\bs(\bR^\trop)$ in $\overline{\cX_\bs(\pos)}$ if and only if $[\log \mathbf{X}^{(v)}(g_n)]$ converges to $[\mathbf{x}^{(v)}(L)]$ in $\bS \bR^I=(\bR^I \setminus \{0\})/\bR_{>0}$  (cf. \cite[Section 7]{Le16}).

For $L \in \cX_\bs(\bR^\trop)$ and $v \in \bExch_\bs$, we define
\begin{align*}
    \cE^+_{(v)}(g_0) := \Big\{ \lim_{t \to \infty} E(g_0,\, t \cdot L)\ \Big|\ L \in \cC^+_{(v)} \Big\} \subset \bS \cX_\bs(\bR^\trop).
\end{align*}

\begin{thm}\label{thm:D_at_bdry}
Under the identification \eqref{eq:iota}, we have
\begin{align*}
    \cE^+_{(v)}(g_0) = \iota^{-1}(\bS \cC^+_{(-v)}) \subset \bS \cX_\bs(\bR^\trop)
\end{align*}
for each $g_0 \in \cX_\bs(\pos)$ and $v \in \bExch_\bs$.
Thus, the set of the faces of $\{\cE^+_{(v)}(g_0) \mid v \in \bExch_\bs\}$ coincides with the cluster complex \cite{FZ-CA2}
%``projectivized" fan
%\footnote{This forms a simplical complex, called \emph{cluster complex} in \cite{FZ-CA2}} 
$\bS \fF^+_{-\bs} := \{ \bS \cC \mid \cC \in \fF^+_{-\bs}\}$ via the identification $\iota$.
\end{thm}
\begin{proof}
% For each $v \in \bExch_\bs$, take a path $\gamma: v_0 \to v$ in $\bExch_\bs$.
Take $v \in \bExch_\bs$.
For $k \in I$, let $L = L^{(v)}_{k} \in \cC_{(v)}^+$ be the elementary lamination characterized by $x_i^{(v)}(L^{(v)}_k) = \delta_{ik}$. Then from the definition, the earthquake along $t \cdot L$ satisfies $X_i^{(v)}(E(g_0,t\cdot L)) = e^{\delta_{ik}t} X_i^{(v)}(g_0)$. 
By using the separation formula \cref{?}, we rewrite it in the coordinate $X_i^{(v_0)}$ as
\begin{align*}
    X_i^{(v_0)}(E(g_0,\, t \cdot L)) 
    &= \Big( \prod_{j \in I} (X_j^{(v)}(E(g_0,\, t \cdot L)))^{c_{ij}} \cdot F_j^{v \to v_0}(\mathbf{X}^{(v)}(E(g_0,\, t \cdot L)))^{\varepsilon^{(v)}_{ij}} \Big)\\
    &= (e^t)^{c_{ik}} \cdot \Big( \prod_{j \in I} (X_j^{(v)}(g_0))^{c_{ij}} \cdot F_j^{v \to v_0}(\mathbf{X}^{(v)}(E(g_0,\, t \cdot L)))^{\varepsilon^{(v)}_{ij}} \Big)
\end{align*}
where $C^{\bs}_{v \to v_0} = (c_{ij})_{i,j \in I}$.
Hence,
\begin{align*}
    \log X_i^{(v_0)}(E(g_0,\, t \cdot L)) &=
    t \cdot c_{ik} +\sum_{j \in I}c_{ij} \log X_j^{(v)}(g_0)
    + \sum_{j \in I} \varepsilon^{(v)}_{ij} \log F^{v \to v_0}_j(\mathbf{X}^{(v)} (E(g_0,\, t \cdot L))).
\end{align*}
Recall that the $F$-polynomial has the following form:
\begin{align}\label{eq:F_exp}
    F_j^{v \to v_0}(\mathbf{X}^{(v)}) = 1 + \sum_{\alpha=(\alpha_m)} \xi_\alpha\cdot \prod_{m \in I} (X_m^{(v)})^{\alpha_m} + \prod_{m \in I} (X_m^{(v)})^{f_{jm}}
\end{align}
for some constants $\xi_\alpha \in \bZ$,
where $F_{v \to v_0}^\bs=(f_{jm})_{j,m \in I}$ is the $F$-matrix (\cref{def:F-mat}), and $\alpha=(\alpha_m)$ runs over certain set of integral vectors satisfying $\alpha_m \leq f_{jm}$ for all $m \in I$. 
Then the last term is estimated as 
\begin{align*}
    &\frac{1}{t}\log F^{v \to v_0}_j(\mathbf{X}^{(v)} (E(g_0,\, t \cdot L))\\
    &\hspace{3cm}= \frac{1}{t}\log F_j^{v \to v_0}(X_1^{(v)}(g_0), \dots, e^t X_k^{(v)}(g_0), \dots, X_N^{(v)}(g_0))\\
    &\hspace{3cm}= \frac{1}{t}\log \Big(1 + \sum_{\alpha} e^{t \cdot \alpha_k}\xi_\alpha\cdot \prod_{m} X_m^{(v)}(g_0)^{\alpha_m} + e^{t \cdot f_{jk}} \prod_{m}X^{(v)}_m(g_0)^{f_{jm}}\Big)\\
    &\hspace{3cm}\xrightarrow[t \to \infty]{} f_{jk},
\end{align*}
%where $F^{\bs}_{v \to v_0} = (f_{ij})_{i,j \in I}$.
since $e^{tf_{jk}}$ is the dominant term inside the logarithm. 
Therefore,
\begin{align*}
    \lim_{t \to \infty} \frac{\log X_i^{(v_0)}(E(g_0,\, t \cdot L))}{t}
    = c_{ik} + \sum_{j \in I} \varepsilon_{ij}^{(v)}f_{jk}.
\end{align*}
By \cite[Theorem 2.8]{FuGy}, we have
\begin{align*}
    C^{\bs}_{v \to v_0} + \varepsilon^{(v)} F^{\bs}_{v \to v_0}
    = C^{-\bs}_{v \to v_0}.
\end{align*}
Thus, $\bS \mathbf{x}^{(v_0)}(\cE_{(v)}^+(g_0))$ is the convex hull in $\bS \mathbf{x}^{(v_0)}(\cX_\bs(\bR^\trop))$ spanned by the points represented by the column vectors of $C_{v \to v_0}^{-\bs} = (G_{v_0 \to v}^\bs)^\tr$.
On the other hand, the cone $x_{(-v_0)}(\cC^+_{(-v)})$ is also spanned by the $g$-vectors from $v_0$ to $v$ at $\bs$ by \cref{prop:cl_cpx=g-vect_fan}.
% of $C^{-\bs}_{v \to v_0}$, since the presentation matrix of the linear map $x_{(-v_0)} \circ x_{(-v)}^{-1}|_{\bR_{\geq 0}^I}$ is the matrix $C^{-\bs}_{v \to v_0}$ by \cite[Lemma 3.12]{IK20}.
Thus these two cones coincides with each other.
\end{proof}




\subsection{The case of $g$ to the boundary}\label{subsec:g_to_infty}
We continue to fix a seed pattern $\bs$ of finite type and a vertex $v_0 \in \bExch_\bs$.
We are going to observe the asymptotic behavior of the subsets $\cD_{(v)}^+(g_0)$ as $g_0$ to the boundary $\bS \cX_\bs(\bR^\trop)$ in $\log \mathbf{X}^{(v_0)}(\cX_\bs(\bR^\trop))$ and we will show that they converge to some cones.

For $g_0 \in \cX_\bs(\pos)$ and $v_0 \in \bExch_\bs$, we define the set $\fG_{(v_0)}^+(g_0)$ in $\bR^I$ as the intersections of the subsets
\begin{align*}
    \cB^+_{(v_0;v)}(g_0) := \bigg\{
    \log \frac{\mathbf{X}^{(v_0)}(g)}{\mathbf{X}^{(v_0)}(g_0)} \, \bigg|\,
    g \in \cD^+_{(v)}(g_0) \bigg\}, \quad v \in \bExch_\bs.
\end{align*}
Since $\log \mathbf{X}^{(v_0)}(g_0) \neq \mathbf{0}$, we took the subtraction $- \log \mathbf{X}^{(v_0)}(g_0)$ in the definition of $\cB^+_{(v_0; v)}(g_0)$.

\begin{thm}
Let $\bs$ be a seed a seed pattern of finite type and $v_0 \in \bExch_\bs$.
% Let $g_y \in \cX_\bs(\pos)$ be satisfying $X^{(v_0)}_i(g_y) = e^y$ for $y \in \bR$ and for all $i \in I$.
Then, 
% \begin{align*}
%     \lim_{y \to \mp \infty} \cG_{(v_0)}(g_y) = \fF^\pm_{(v_0)}\,.
% \end{align*}
\begin{align*}
    % \lim_{\mathbf{X}^{(v_0)}(g)^{\pm 1} \to \mathbf{0}} \fG^+_{(v_0)}(g) = \mathbf{x}^{(v_0)}(\fF^\mp_{\bs})\,.
    \fG^+_{(v_0)}(g_0) \to x_{(\pm v_0)}(\fF^+_{\pm \bs}) \quad \mbox{as $g_0$ diverges to $\interior \bS \cC^\pm_{(v_0)}$}.
\end{align*}
Namely, the subsets $\cB^+_{(v_0;v)}(g_0)$ converge to $x_{(\pm v_0)}(\cC^+_{(\pm v)})$ in the Gromov--Hausdorff sense as $g_0  \in \cX_\bs(\pos)$ diverges so that $\mathbf{X}^{(v_0)}(g_0)^{\mp 1} = (X^{(v_0)}_i (g_0)^{\mp 1})_{i \in I} \to \mathbf{0}$.
\end{thm}

\begin{proof}
For $v \in \bExch_\bs$ and $L \in \cC^+_{(v)}$, we put $T_i := \exp(x^{(v)}_i(L))$.
Let us put
% $\gamma:v_0 \to v$ in $\bExch_\bs$, 
$C^\bs_{v \to v_0} = (c_{ij})_{i,j \in I}$ and $F^\bs_{v \to v_0} = (f_{ij})_{i,j\in I}$.
Then, for any $g \in \cX_\bs(\pos)$, by the separation formula \cref{thm:sep_for},
\begin{align*}
    X_i^{(v_0)}(E(g, L))
    &= \prod_{j \in I} X_j^{(v)}(E(g, L))^{c_{ij}} \cdot F_j^{v \to v_0} (\mathbf{X}^{(v)}(E(g, L)))^{\varepsilon_{ij}^{(v)}}\\
    &=\Big(\prod_{j \in I} T_j^{\,c_{ij}}\Big) \cdot \Big(\prod_{j \in I} (X_j^{(v)}(g))^{c_{ij}} \cdot F_j^{v \to v_0}(T \cdot \mathbf{X}^{(v)}(g))^{\varepsilon^{(v)}_{ij}}\Big),
\end{align*}
where $T \cdot \mathbf{X}^{(v)} = (T_i \cdot X_i^{(v)})_{i \in I}$.
Let $L^{(v)}_i \in \cC^+_{(v)}$ be a point satisfying $x^{(v)}_j(L^{(v)}_i) = \delta_{ij}$.
Then, we have
\begin{align*}
    \log \frac{X_i^{(v_0)}(E(g, L^{(v)}_k))}{X_i^{(v_0)}(g)}
    &=
    c_{ik} + \sum_{j \in I}
    \varepsilon_{ij}^{(v)} \log \frac{F_j^{v \to v_0}(T \cdot \mathbf{X}^{(v)}(g))}{F_j^{v \to v_0}(\mathbf{X}^{(v)}(g))}.
\end{align*}
By \eqref{eq:F_exp}, we have
\begin{align}
    \log \frac{F_j^{v \to v_0}(T \cdot \mathbf{X}^{(v)}(g))}{F_j^{v \to v_0}(\mathbf{X}^{(v)}(g))}
    &= \log \frac{1 + \sum_{\alpha} \xi_\alpha e^{\alpha_k} \cdot \prod_{\ell \in I} X_\ell^{(v)}(g)^{\alpha_\ell} + e^{f_{jk}} \prod_{\ell \in I} X_\ell^{(v)}(g)^{f_{j\ell}}}{1 + \sum_{\alpha} \xi_\alpha\cdot \prod_{\ell \in I} X_\ell^{(v)}(g)^{\alpha_\ell} + \prod_{\ell \in I} X_\ell^{(v)}(g)^{f_{j\ell}}}\label{eq:log_frac_F}\\
    &= \log \frac{\prod_{\ell \in I} X_\ell^{(v)}(g)^{-f_{j\ell}} + \sum_{\alpha}\xi_\alpha e^{\alpha_k} \cdot \prod X_\ell^{(v)}(g)^{\alpha_\ell - f_{j\ell}} + e^{f_{jk}}}{\prod_{\ell \in I} X_\ell^{(v)}(g)^{-f_{j\ell}} + \sum_{\alpha}\xi_\alpha \cdot \prod X_\ell^{(v)}(g)^{\alpha_\ell - f_{j\ell}} + 1}.\label{eq:log_frac_F_inv}
\end{align}
Moreover, we have
\begin{align}\label{eq:X_(v)}
    X_\ell^{(v)}(g) = 
    \prod_{m \in I} X_m^{(v_0)}(g)^{\overline{c}_{\ell m}} \cdot F_m^{v_0 \to v}(\mathbf{X}^{(v_0)}(g))^{\varepsilon^{(v_0)}_{\ell m}}
\end{align}
where $C^\bs_{v_0 \to v} = (\overline{c}_{ij})_{i,j \in I}$.
Since $F_m^{v_0 \to v}(\mathbf{X}^{(v_0)}(g))$ is a polynomial in $\mathbf{X}^{(v_0)}(g)$, we have
\begin{align*}
    X_\ell^{(v)}(g) \sim \prod_{m \in I} X_m^{(v_0)}(g)^{\overline{c}_{\ell m}} \quad \mbox{as } \mathbf{X}^{(v_0)}(g) \to \mathbf{0}.
\end{align*}
By \cref{cor:FC_non-pos_fin}, $-\sum_\ell f_{j \ell} \oline{c}_{\ell m} > 0$.
Hence, by the expression \eqref{eq:log_frac_F_inv}, we have
\begin{align*}
    \lim_{\mathbf{X}^{(v_0)}(g) \to \mathbf{0}} \log \frac{F_j^{v \to v_0}(T \cdot \mathbf{X}^{(v)}(g))}{F_j^{v \to v_0}(\mathbf{X}^{(v)}(g))} = f_{jk}.
\end{align*}
% and \cite{NZ}, $\eqref{eq:log_frac_F} \to 0$ as $\mathbf{X}^{(v_0)}(g) \to \mathbf{0}$.
Therefore, by \cite{FuGy},
\begin{align*}
    \lim_{\mathbf{X}^{(v_0)}(g) \to \mathbf{0}} \bigg(
    \log \frac{X_i^{(v_0)}(E(g, L^{(v)}_k))}{X_i^{(v_0)}(g)}
    \bigg)_{i,k \in I}
    = C^{\bs}_{v \to v_0} + \varepsilon^{(v)} F^\bs_{v \to v_0}
    = C^{-\bs}_{v \to v_0}
    = (G^{\bs}_{v_0 \to v})^\tr.
\end{align*}
By \cref{prop:cl_cpx=g-vect_fan}, we get $\lim_{\mathbf{X}^{(v_0)}(g) \to \mathbf{0}} \fG^+_{(v_0)}(g) = x_{(-v_0)}(\fF^+_{-\bs})$.
On the other hand, by \cite[Proposition 5.3]{FZ-CA4}, we have
\begin{align*}
    F_{m}^{v_0 \to v}(\mathbf{X}^{(v_0)}(g)) = 
    \prod_{p \in I} X_p^{(v_0)}(g)^{\overline{f}_{mp}} \cdot \check{F}_m^{v_0 \to v}(\mathbf{X}^{(v_0)}(g)^{-1})
\end{align*}
where $F_{v_0 \to v}^\bs = (\overline{f}_{ij})_{i,j \in I}$ and 
$\check{F}^{v_0 \to v}_m$ be the $m$-th $F$-polynomial from $v_0$ to $v$ in the opposite mutation class $-\bs$.
By \cite[Theorem 2.8]{FuGy},
\begin{align*}
    C^\bs_{v_0 \to v} + \varepsilon^{(v_0)} F^\bs_{v_0 \to v} = C^{-\bs}_{v_0 \to v}.
\end{align*}
Thus, in contradistinction to \eqref{eq:X_(v)},
\begin{align*}
    X_\ell^{(v)}(g) \sim
    \prod_{m \in I} X_m^{(v_0)}(g)^{\check{c}_{\ell m}} \quad \mbox{as } \mathbf{X}^{(v)}(g)^{-1} \to \mathbf{0}
\end{align*}
where $C^{-\bs}_{v_0 \to v} = (\check{c}_{ij})_{i,j \in I}$.
By \cref{cor:FC_non-pos_fin}, $\sum_\ell f_{j \ell} \check{c}_{\ell m} < 0$.
Hence, by the expression \eqref{eq:log_frac_F}, we have
% and \cite{NZ}, $\eqref{eq:log_frac_F} \to f_{jk}$ as $\mathbf{X}^{(v_0)}(g)^{-1} \to \mathbf{0}
\begin{align*}
    \lim_{\mathbf{X}^{(v_0)}(g) \to \mathbf{0}} \log \frac{F_j^{v \to v_0}(T \cdot \mathbf{X}^{(v)}(g))}{F_j^{v \to v_0}(\mathbf{X}^{(v)}(g))} = 0.
\end{align*}
% Thus, 
% \begin{align*}
%     \eqref{eq:log_frac_F} = 
%     \log \frac{\prod_{\ell \in I} X_\ell^{(v)}(g)^{-f_{j\ell}} + \sum_{\alpha}\xi_\alpha e^{\alpha_k} \cdot \prod X_\ell^{(v)}(g)^{\alpha_\ell - f_{j\ell}} + e^{f_{jk}}}{\prod_{\ell \in I} X_\ell^{(v)}(g)^{-f_{j\ell}} + \sum_{\alpha}\xi_\alpha \cdot \prod X_\ell^{(v)}(g)^{\alpha_\ell - f_{j\ell}} + 1}.
% \end{align*}
Therefore, 
\begin{align*}
    \lim_{\mathbf{X}^{(v_0)}(g)^{-1} \to \mathbf{0}} \bigg(
    \log \frac{X_i^{(v_0)}(E(g, L^{(v)}_k))}{X_i^{(v_0)}(g)}
    \bigg)_{i,k \in I}
    = C_{v \to v_0}^\bs
    % = (C_{v_0 \to v}^{-\bs})^{-1}
    = (G_{v_0 \to v}^{-\bs})^\tr.
\end{align*}
By \cref{prop:cl_cpx=g-vect_fan}, we get $\lim_{\mathbf{X}^{(v_0)}(g)^{-1} \to \mathbf{0}} \fG^+_{(v_0)}(g) = \mathbf{x}^{(v_0)}(\fF^+_{\bs})$.
\end{proof}

This theorem describes the asymptotics of the simplical set $\fG^+_{(v_0)}(g_0)$ in the direction only $\interior \bS \cC^\pm_{(v_0)}$.
We conclude this subsection with the following problem:
\begin{prob}
Describe the asymptotic behavior of $\fG^+_{(v_0)}(g_0)$ when $g_0$ goes to the boundary $\bS \cX_\bs(\bR^\trop)$ except the subsets $\interior \bS \cC^\pm_{(v_0)}$.
\end{prob}


